Unconventional Superconductivity and Magnetism in Lanthanide and Actinide Intermetallic Compounds

In this review article we present a survey of unconventional superconductors and their coexistence behaviour with magnetism. We focus on Ce- and U-based heavy fermion superconductors, in addition we discuss the rare earth borocarbide and skutterudite superconductors. We show that heavy fermion behaviour in Ce- and U- compounds should be described differently. While the Kondo-lattice model with localised 4f-electrons is appropriate for Ce-compounds, dual models including localised and itinerant 5f-electrons are necessary for U-compounds. We demonostrate that this leads to consistent results for Fermi surface topology and mass enhancement in various U-compounds. We also show that virtual exchange of localised 5f-electron excitations provides a new mechanism for unconventional superconductivity in addition to the known itinerant spin-fluctuation exchange mechanism. We discuss symmetry properties and coexistence of unconventional superconducting and density wave (hidden) order parameters and methods for their detection, notably the new angle resolved magntetotransport methods. The latter have been very succesful for the investigtion of gap anisotropies in the nonmagnetic borocarbide superconductors. Recent results on the new multiphase Pr-skutterudite superconductor are also reviewed.

==> 0subject.tex <==
%auto-ignore
\twocolumn
{\em subject index entries}\\[0.5cm]
\begin{itemize}
\item antiferromagnetic order
\item antiferroquadrupolar order
\item band structure
\item BCS ratio
\item Blount's theorem
\item borocarbides
\item B-T phase diagram
\item CeCoIn$_5$
\item CeCu$_2$Si$_2$
\item CeCu$_2$Ge$_2$
\item CeCu$_2$(Si$_{1-x}$Ge$_x$)$_2$
\item CeIrIn$_5$
\item CeMIn$_5$
\item CeM$_2$X$_2$
\item CePd$_2$Si$_2$
\item CeNi$_2$Ge$_2$
\item CeRhIn$_5$
\item CeRh$_2$Si$_2$
\item Ce$_2$RhIn$_8$
\item CeRu$_2$Si$_2$
\item CeRu$_2$Ge$_2$
\item RNi$_2$B$_2$C
\item CePt$_3$Si
\item charge density wave
\item coexistence
\item conventional pairing
\item Coulomb interaction
\item crystalline electric field excitations
\item de Haas-van Alphen effect
\item Doppler shift
\item dual model
\item d-wave gap
\item DyNi$_2$B$_2$C
\item E$_{2u}$-model
\item effective interaction
\item electron-electron pairing
\item electron-hole pairing
\item electron-phonon superconductivity
\item Eliashberg equations
\item ErNi$_2$B$_2$C
\item Fermi liquid
\item Fermi liquid parameters
\item Fermi surface
\item Fermi velocity
\item Fermi wave vector
\item ferromagnetic order
\item FFLO phase
\item form factor
\item free energy
\item gap function
\item gap equations
\item gap nodes
\item giant diamagnetism
\item Ginzburg-Landau theory
\item heavy fermions
\item hidden order
\item high-T$_c$
\item HoNi$_2$B$_2$C
\item Hubbard model
\item Hund's rules
\item hybridisation
\item hydrostatic pressure
\item incommensurate order
\item induced moment magnetism
\item inelastic neutron scattering
\item impurity scattering
\item jj-coupling
\item Knight shift
\item Kondo lattice
\item Kondo resonance
\item Kondo temperature
\item Landau levels
\item Landau parameters
\item LaRu$_2$Si$_2$
\item LuNi$_2$B$_2$C
\item magnetic exciton
\item magnetotransport
\item magnetostriction
\item mass enhancement
\item metamagnetism
\item multiphase superconductivity
\item nesting property
\item neutron diffraction
\item non-Fermi liquid state
\item nuclear magnetic resonance
\item order parameter
\item phase shifts
\item point nodes
\item power laws
\item PrOs$_4$Sb$_{12}$
\item quantum critical point
\item quasiparticle excitations
\item quasiparticle DOS
\item quasiparticle tunneling
\item reentrance behaviour
\item RKKY interaction
\item RNi$_2$B$_2$C
\item singlet CEF state
\item singlet pairing
\item skutterudites
\item s+g wave gap
\item skutterudites
\item spin density wave
\item spin fluctuation
\item spin orbit coupling
\item specific heat
\item strong coupling effects
\item superclean limit
\item susceptibility 
\item symmetry group
\item T$_c$-splitting
\item tetracritical point
\item thermal conductivity
\item thermal expansion
\item Th$_{1-x}$U$_x$Ru$_2$Si$_2$
\item tight binding model
\item time reversal symmetry
\item triplet pairing
\item UBe$_{13}$
\item UGe$_2$
\item unconventional pairing
\item unitary state
\item ultrasonic attenuation
\item upper critical field
\item UNi$_2$Al$_3$
\item UPd$_2$Al$_3$
\item UPt$_3$
\item URu$_2$Si$_2$
\item U$_{1-x}$Th$_x$Be$_{13}$
\item Volovik effect
\item Wiedemann-Franz law
\item vortex phase
\item x-T phase diagram
\item YNi$_2$B$_2$C
\item Y(Ni$_{1-x}$Pt$_x$)$_2$B$_2$C
\item YbRh$_2$Si$_2$
\end{itemize}
\onecolumn
